Prompted Contextual Vectors for Spear-Phishing Detection

Spear-phishing attacks present a significant security challenge, with large language models (LLMs) escalating the threat by generating convincing emails and facilitating target reconnaissance. To address this, we propose a detection approach based on a novel document vectorization method that utilizes an ensemble of LLMs to create representation vectors. By prompting LLMs to reason and respond to human-crafted questions, we quantify the presence of common persuasion principles in the email's content, producing prompted contextual document vectors for a downstream supervised machine learning model. We evaluate our method using a unique dataset generated by a proprietary system that automates target reconnaissance and spear-phishing email creation. Our method achieves a 91\% F1 score in identifying LLM-generated spear-phishing emails, with the training set comprising only traditional phishing and benign emails. Key contributions include a novel document vectorization method utilizing LLM reasoning, a publicly available dataset of high-quality spear-phishing emails, and the demonstrated effectiveness of our method in detecting such emails. This methodology can be utilized for various document classification tasks, particularly in adversarial problem domains.

==> algorithms/dataset_creation_algo.tex <==
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{amsmath}

\begin{algorithm}
\caption{Constructing Dataset from Emails}
\begin{algorithmic}[1]
\State $ \text{dataset} = []$
\For {every email $e$}
    \State $ \text{email\_vector} = []$
    \For {every question $q$}
        \For {every language model $l$}
            \State $ \text{probability} = \text{ask\_question}(e, q, l)$ 
            \State $ \text{email\_vector.append(probability)}$
        \EndFor
    \EndFor
    \State $ \text{dataset.append(email\_vector)}$
\EndFor
\end{algorithmic}
\end{algorithm}


==> tables/mistral_ablation.tex <==
\begin{table*}[t]
  \centering
  \caption{LLM ensemble ablation study results}
  \begin{tabular}{lccccc}
    \toprule
    \textbf{LLMs Ensemble} & \textbf{Recall} & \textbf{Precision} & \textbf{F1} & \textbf{Geometric Mean} & \textbf{False Positive Rate (FPR)} \\
    \midrule
    Mistral Large, Mistral Small & 0.93 & 0.71 & 0.8 & 0.9 & 0.13 \\
    Mistral Large & 0.93 & 0.66 & 0.77 & 0.88 & 0.16 \\
    Mistral Small & 0.87 & 0.48 & 0.62 & 0.77 & 0.31 \\
    \bottomrule
  \end{tabular}
  \label{tab:ablation_results}
\end{table*}
